Humane Visual AI: Telling the Stories Behind a Medical Condition

A biological understanding is key for managing medical conditions, yet psychological and social aspects matter too. The main problem is that these two aspects are hard to quantify and inherently difficult to communicate. To quantify psychological aspects, this work mined around half a million Reddit posts in the sub-communities specialised in 14 medical conditions, and it did so with a new deep-learning framework. In so doing, it was able to associate mentions of medical conditions with those of emotions. To then quantify social aspects, this work designed a probabilistic approach that mines open prescription data from the National Health Service in England to compute the prevalence of drug prescriptions, and to relate such a prevalence to census data. To finally visually communicate each medical condition's biological, psychological, and social aspects through storytelling, we designed a narrative-style layered Martini Glass visualization. In a user study involving 52 participants, after interacting with our visualization, a considerable number of them changed their mind on previously held opinions: 10% gave more importance to the psychological aspects of medical conditions, and 27% were more favourable to the use of social media data in healthcare, suggesting the importance of persuasive elements in interactive visualizations.

==> Humane AI for Health/prescriptions.tex <==
\subsection{Quantifying Social Aspects}\label{quantifying-prescriptions}
% \begin{figure}[t!]
%     \centering
%     \includegraphics[width=\columnwidth]{Linking.pdf}
%     \caption{
%         The four NHS Datasets: \emph{(a)} NHS GP monthly prescriptions; \emph{(b)} NHS drugs; \emph{(c)} NHS GPs; and \emph{(d)} NHS patients. Each monthly prescription in dataset \emph{(a)} was translated into a drug name based on the BNF code for which dataset \emph{(b)} offered the corresponding drug (preparation name). The prescription was also geographically mapped using the GP code for which dataset \emph{(c)} provided the location.  To then map the prescription at the level of census LSOAs, we computed the fraction of the GP's patients who lived in each LSOA from dataset  \emph{(d)}.}
%     \label{Fig:data_link}
% \end{figure}
People's social environment can cause or affect their health. For example, the economic status has an influence on people's diets, and this, in turn, can affect whether they will suffer from diabetes \cite{aiello2019large}. On the other hand, people's medical condition can influence their social life -- for instance, cancer patients experiencing severe pain are likely to suffer from lowered-self esteem and anxiety \cite{ozdemiroglu2017self}. 
To associate socio-economic conditions with disease prevalence, we associated census data with prescription data across all the boroughs in England.
%To quantify social aspects of medical conditions, we looked at their geographic distribution, i.e., prevalence across different boroughs. In this way, we could capture and quantify the relationship of the deprivation scores, population, and population density with the prevalence of conditions. 

Prescription data is released by the National Health Service (NHS)
and enumerates all the prescriptions done by any general practice (GP) across England. 
The drug prescription data has been made  available since July 2010, is released every month by NHS~\cite{BNFsummary}, and consists of four files (Figure S2 the Supplemental Material), which we collected  until the end of June 2019:
i) \emph{NHS GP monthly prescriptions:} each prescription contains the drug's name, its  British National Formulary (BNF) code, the practice code, its total number of items, total cost, and each item's quantity; ii) \emph{NHS drugs:} each row contains a drug (individual preparation name) and its unique BNF Code; iii) \emph{NHS GPs:} each row contains a practice code, name, and full address; and iv) \emph{NHS GP patients:} each row contains a practice code, census LSOA borough code (each row refers to a specific (practice, LSOA) pair), and the number of the practice's patients in that borough. From this file, we  computed the total number of primary care patients who live in each borough.

% \begin{description}[leftmargin=*]
%     \itemsep0em 
%     \item \emph{NHS GP monthly prescriptions}, Figure Figure S2\emph{(a)}. These are  all the  \emph{anonymized} prescriptions during a month in the whole England. Each prescription contains the drug's name, its BNF code, the practice code, its total number of items, total cost, and each item's quantity (i.e., number of pills and their potency, volume of liquid in ml. etc.). 
    
%     \item \emph{NHS drugs}, Figure S2\emph{(b)}. Each row contains a drug (individual preparation name) and its unique British National Formulary (BNF) Code~\cite{BNFglossary}. There are 2921 distinct drug names in total. 
%     % BNF code here is truncated 
    
%     \item \emph{NHS GPs}, Figure S2\emph{(c)}. Each row contains a practice code (its unique identifier), name, and full address. The file contains 9905 GPs, from which we filter away those that are closed or hosted in prisons, leaving us with 6924 GPs across England. 
    
%     \item \emph{NHS GP patients}, Figure S2\emph{(d)}. Each row contains a practice code, census LSOA borough code (each row refers to a specific (practice,LSOA) pair), and the number of the practice's patients in that borough~\cite{patientregistry}. From this file, we  computed the total number of primary care patients who live in borough $a$: $N_{patients@a} = \sum_{GP} N_{patients@GP,a}$,
%     where $N_{patients@GP,a}$ is the number of $GP$'s patients who live in $a$. We also  computed the corresponding \emph{fraction} of patients:
%     $
%     F_{patients@GP,a} = \frac{ N_{patients@GP,a}  } { N_{patients@GP} }
%     $
% \end{description}


The data, however, does not contain any mapping between the prescribed drugs and the corresponding medical conditions. To create such a mapping, we crawled the entire database from DrugBank\footnote{\url{drugbank.ca}}. From the database, we obtained $9105$ drug-related pages. Out of those, we were able to match $3013$ to at least one associated condition. This gave us a mapping between drugs and conditions. More specifically, for a given condition $C$, we used DrugBank to find the set of drugs $D$ associated with it to then estimate the total prescriptions related to $C$ in a borough $A$.

%For every borough $A$ and condition $C$, we calculated the prevalence confidence ($conf_A$). {More details on this calculation are provided in the Supplemental Material document.}

% For a given condition $C$, we used DrugBank to find a set of drugs $D$ that are associated as a treatment for condition $C$. We then estimate the total number of prescriptions given by all the GPs in a borough $a$ as: 
% $
% & N_{C@a}  = \sum_{j \in D}\sum_{GP} N_{j@GP}  \cdot F_{patients@GP,a},
% $
% where $j$ is a drug name from the list of drugs $D$, associated with $C$, and $N_{j@GP}$ are the total number of prescriptions written for drug $j$ at the $GP$. $N_{C@a}$ is the total number of $C$ related prescriptions written in a borough.
% We normalized this quantity by 1000 patients, as it is typically done in medical studies~\cite{curtis2018openprescribing,curtis2019opioid}:
% $
% Norm_{j@a} =\frac{ N_{j@a} }{ N_{patients@a}  } \cdot 1000
% $, where $Norm_{j@a}$ is our prescription based prevalence for condition $C$ at borough $a$.

% Our way of  counting the number of prescription items has one major drawback though: each prescription item is counted as one no matter how strong its dosage (number of pills) and potency (milligrams or micro-grams) are. This drawback is common in the literature: previous studies mainly considered simple item count and discarded dosage information because it is hard to consider that information when processing prescriptions manually~\cite{curtis2018openprescribing}. Another way of normalizing prescriptions entails the use of  the Defined Daily Dosage\cite{whoDDD}, which 
% defines an average maintenance dose  for a drug  for a typical adult per day. Unfortunately, these dosages are not defined for all the drugs in the NHS dataset. Therefore, we needed a method that could work for all the drugs. Fortunately, being able to  mine prescriptions automatically made it possible for us to go beyond item count or Defined Daily Dosage. Indeed, to account for both dosage and potency, we introduced the concept of  \emph{dosage unit} and computed it for each prescribed drug. This quantity reflects the extent to which the drug departed from its minimum dosage (e.g., 2 units for a prescribed drug mean that the prescribed drug's dosage and potency are twice its potential minimum). Mathematically:
% \begin{equation*}
%     \begin{aligned}
%         Unit_{prescribed}  =\frac{ Dosage_{prescribed} }{ min (Dosage_{drug}) } 
%         \cdot \frac{ Potency_{prescribed} } {min(Potency_{drug})}
%     \end{aligned}
% \end{equation*} 
% where $Dosage_{prescribed} $ and $Potency_{prescribed} $ are the dosage and potency of  the prescribed drug, and  $min(Dosage_{drug})$ and \break $min(Potency_{drug})$ are the minimum dosage and potency of that drug across other prescriptions of it. The denominators are normalization factors that make the dosages of different drugs comparable. To ease understanding, consider $GP J82120$ who prescribed  120 pills of the anti-heart burn drug Ranitidine 150mg. By sorting through all the prescriptions of Ranitidine, our framework found  that the minimum potency tablet is of 5mg, and the minimum quantity is 2 pills; therefore, by using these values at the two denominators, we found the dosage of the prescribed drug to be $Unit_{prescribed} = \frac{120}{2} \cdot \frac{150}{5}=1800$. 
% By then converting all the prescriptions in terms of dosage units, we estimated the dosage of the prescriptions for all the patients who lived in borough $a$ with formula~(\ref{eq:items:condition}) in which $j=dosage$, and $N_{j@GP} $ is the total dosage of $GP$'s prescriptions computed by summing up the dosage units for all $GP$'s prescriptions:
% \begin{equation}
% N_{dosage@GP}   = \sum_{prescribed @ GP} Unit_{prescribed}
% \end{equation}
% Once the normalized dosage per GP is obtained, we can then estimate the prescription based prevalence at an borough $a$ by substituting the value of $N_{dosage@GP}$ in equation \ref{eq:items:condition}

% Since our approach is probabilistic, for every borough level condition prevalence, we also generated a \textit{confidence score}. For any given condition $C$, we first calculated mean and standard deviation of the prescription prevalence (calculated above) across all the borough councils of England, for any given condition $C$. Let $\mu^{UK}_c$ and $\sigma^{UK}_c$ be the mean and standard deviation for the log transformed number of prescription prevalence for a condition $C$ across all the boroughs of England. 
% Let $\mu^{UK}$ and $\sigma^{UK}$ be the mean and standard deviation for the log of total inclusive number of all prescription prevalences across all the boroughs of England. 
% Let $P^d_A$ be the log of total number of $C$-related prescription prevalence at borough A. Also, let $P_A$ be the log of total number of all inclusive prescription prevalence at borough A.  
% We then defined two windows of confidence:  $window^d_A= P^d_A - \mu^{UK}_d + n \cdot\sigma^{UK}_d $ and $window_A= P_A - \mu^{UK} + \hat{n} \cdot\sigma^{UK}$ 
% We chose the value of $n = 2$ and $\hat{n} = 2$. From this, for any borough $A$ we calculated the prevalence confidence as: 
% \begin{equation}
%   conf_A =  \begin{cases}
%                       0                          & \text{if $ window_A < 0$ and $window^d_A < 0$}.\\
%                       1-\frac{1}{(window^d_A+1)} & \text{otherwise}.
%                     \end{cases}
% \end{equation}
